MTV-Inpaint: Multi-Task Long Video Inpainting

Video inpainting involves modifying local regions within a video, ensuring spatial and temporal consistency. Most existing methods focus primarily on scene completion (i.e., filling missing regions) and lack the capability to insert new objects into a scene in a controllable manner. Fortunately, recent advancements in text-to-video (T2V) diffusion models pave the way for text-guided video inpainting. However, directly adapting T2V models for inpainting remains limited in unifying completion and insertion tasks, lacks input controllability, and struggles with long videos, thereby restricting their applicability and flexibility. To address these challenges, we propose MTV-Inpaint, a unified multi-task video inpainting framework capable of handling both traditional scene completion and novel object insertion tasks. To unify these distinct tasks, we design a dual-branch spatial attention mechanism in the T2V diffusion U-Net, enabling seamless integration of scene completion and object insertion within a single framework. In addition to textual guidance, MTV-Inpaint supports multimodal control by integrating various image inpainting models through our proposed image-to-video (I2V) inpainting mode. Additionally, we propose a two-stage pipeline that combines keyframe inpainting with in-between frame propagation, enabling MTV-Inpaint to effectively handle long videos with hundreds of frames. Extensive experiments demonstrate that MTV-Inpaint achieves state-of-the-art performance in both scene completion and object insertion tasks. Furthermore, it demonstrates versatility in derived applications such as multi-modal inpainting, object editing, removal, image object brush, and the ability to handle long videos. Project page: https://mtv-inpaint.github.io/.

==> tmp.tex <==
To address this issue, we propose the \textbf{K2V prior noise initialization} algorithm. Instead of sampling from random noise, our method initializes the noise by leveraging prior information from the known first and last frames in the sequence.

Formally, let $\mathbf{x}^{k_1:k_2} = \{\hat{\mathbf{x}}^{k_1}, \mathbf{x}^{k_1+1}, \dots, \mathbf{x}^{k_2-1}, \hat{\mathbf{x}}^{k_2}\}$ denote a sequence of interval frames bounded by two known adjacent keyframes $\hat{\mathbf{x}}^{k_1}$ and $\hat{\mathbf{x}}^{k_2}$. We define $\mathcal{P}(\mathbf{x}^i, \mathbf{m}^i)$ as the operation that extracts and resizes the local regions of $\mathbf{x}^i$ specified by $\mathbf{m}^i$ to the median size.

First, the local target regions of the intermediate frames are determined through linear interpolation in the extracted regions:
\[
\mathcal{P}(\hat{\mathbf{x}}^i, \mathbf{m}^i) = (1 - \eta) \mathcal{P}(\hat{\mathbf{x}}^{k_1}, \mathbf{m}^i) + \eta \mathcal{P}(\hat{\mathbf{x}}^{k_2}, \mathbf{m}^i), \quad \eta = \frac{i - k_1}{k_2 - k_1}.
\]

The interpolated regions, $\mathcal{P}(\hat{\mathbf{x}}^i, \mathbf{m}^i)$, are then resized and pasted back into the corresponding regions of $\mathbf{x}^i$ to produce the updated frame $\hat{\mathbf{x}}^i$, which incorporates prior information from the keyframes.

